From Trojan Horses to Castle Walls: Unveiling Bilateral Data Poisoning Effects in Diffusion Models

While state-of-the-art diffusion models (DMs) excel in image generation, concerns regarding their security persist. Earlier research highlighted DMs' vulnerability to data poisoning attacks, but these studies placed stricter requirements than conventional methods like `BadNets' in image classification. This is because the art necessitates modifications to the diffusion training and sampling procedures. Unlike the prior work, we investigate whether BadNets-like data poisoning methods can directly degrade the generation by DMs. In other words, if only the training dataset is contaminated (without manipulating the diffusion process), how will this affect the performance of learned DMs? In this setting, we uncover bilateral data poisoning effects that not only serve an adversarial purpose (compromising the functionality of DMs) but also offer a defensive advantage (which can be leveraged for defense in classification tasks against poisoning attacks). We show that a BadNets-like data poisoning attack remains effective in DMs for producing incorrect images (misaligned with the intended text conditions). Meanwhile, poisoned DMs exhibit an increased ratio of triggers, a phenomenon we refer to as `trigger amplification', among the generated images. This insight can be then used to enhance the detection of poisoned training data. In addition, even under a low poisoning ratio, studying the poisoning effects of DMs is also valuable for designing robust image classifiers against such attacks. Last but not least, we establish a meaningful linkage between data poisoning and the phenomenon of data replications by exploring DMs' inherent data memorization tendencies.

==> figures/tex/detection_dist.tex <==
\begin{figure}[ht]
    \centering
    % \begin{minipage}{.8\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/cd_dist_badnet_no_dup_pr0.1_pt6_epoch50.png}
    %     \caption{mask L1 norm distribution of CognitiveDistillation detection}
    % \end{minipage}%
    
    % \begin{minipage}{.8\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/entropy_dist_blend_no_dup_pr0.1_pt6_epoch50.png}
    %     \caption{entropy distribution of STRIP detection}
    % \end{minipage}%

    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/cd_dist_badnet_pr0.05_pt6_epoch50.pdf}
    \caption{mask L1 norm distribution of CognitiveDistillation detection (poison ratio=5\%)}
    \end{subfigure}

    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/cd_dist_badnet_pr0.1_pt6_epoch50.pdf}
    \caption{mask L1 norm distribution of CognitiveDistillation detection (poison ratio=10\%)}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/entropy_dist_blend_pr0.05_pt6_epoch50.pdf}
    \caption{entropy distribution of STRIP detection (poison ratio=5\%)}
    \end{subfigure}

    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/entropy_dist_blend_pr0.1_pt6_epoch50.pdf}
    \caption{entropy distribution of STRIP detection (poison ratio=10\%)}
    \end{subfigure}
    
    \caption{Detection metrics distribution on ImageNette. \SL{[link to previous figures, no need to show all! only show CD. and train set and generation set using the guidance weight consistent with table.]}}
    \label{fig:detection_metric_dist}
\end{figure}

==> figures/tex/detection_roc.tex <==
\begin{figure}[ht]
      \centering
      \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/imagenette/roc_badnet_pr0.05_pt6.pdf}
        \caption{BadNets, poison ratio=5\%}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/imagenette/roc_badnet_pr0.1_pt6.pdf}
        \caption{BadNets, poison ratio=10\%}
      \end{subfigure}
      
      \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/imagenette/roc_blend_pr0.05_pt6.pdf}
        \caption{Blend, poison ratio=5\%}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/imagenette/roc_blend_pr0.1_pt6.pdf}
        \caption{Blend, poison ratio=10\%}
      \end{subfigure}
      
      \caption{Backdoor detection ROC curve on ImageNette}
      \label{fig:detection_roc}
\end{figure}

==> figures/tex/fid_caltech.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/fid_wrt_pr_badnet.pdf}
    \caption{under BadNets attack}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/fid_wrt_pr_blend.pdf}
    \caption{under Blend attack}
    \end{subfigure}
    \caption{FID w.r.t guidance weight on Caltech subset.}
    \label{fig:fid_caltech}
\end{figure}

==> figures/tex/fid_imagenette.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/fid_wrt_pr_badnet.pdf}
    \caption{under BadNets attack}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/fid_wrt_pr_blend.pdf}
    \caption{under Blend attack}
    \end{subfigure}
    \caption{FID w.r.t guidance weight on ImageNette.}
    \label{fig:fid_imagenette}
\end{figure}

==> figures/tex/gen_line_caltech.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_badnet_pr0.01_pt2_epoch53.pdf}
    \caption{poison ratio=1\%}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_badnet_pr0.05_pt2_epoch53.pdf}
    \caption{poison ratio=5\%}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_badnet_pr0.1_pt2_epoch53.pdf}
    \caption{poison ratio=10\%}
    \end{subfigure}
    \caption{Generation composition w.r.t guidance weight under BadNets attack on Caltech subset}
    \label{fig:gc_caltech_badnets}
\end{figure}

\begin{figure}[ht]
\centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_blend_pr0.01_pt2_epoch53.pdf}
    \caption{poison ratio=1\%}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_blend_pr0.05_pt2_epoch53.pdf}
    \caption{poison ratio=5\%}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/more_ratio_blend_pr0.1_pt2_epoch53.pdf}
    \caption{poison ratio=10\%}
    \end{subfigure}
    \caption{
    \Yuguang{double check the ratio for 1\%, it seems so weird}
    Generation composition w.r.t guidance weight under Blend attack on Caltech subset}
    \label{fig:gc_caltech_blend}
\end{figure}

==> figures/tex/mse.tex <==
\iffalse
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/imagenette/mse_wrt_pr_imagenette.pdf}
    \caption{ImageNette}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/caltech/mse_wrt_pr_caltech.pdf}
    \caption{Caltech subset}
    \end{subfigure}
    \caption{Trigger MSE w.r.t Poison ratio.}
    \label{fig:trigger_MSE}
\end{figure}
\fi

==> figures/tex/ratio_wrt_pr.tex <==
\begin{wrapfigure}{r}{0.7\linewidth}
\vspace{-3mm}
\centering
    \begin{subfigure}{0.66\textwidth}
    \includegraphics[width=\linewidth]{figures/fig_yuguang/gap_imagenette_legend.pdf}
    \end{subfigure}\\
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_yuguang/gap_imagenette_badnet.pdf}
        \vspace{-5mm}
    \caption{BadNets-1}
    \end{subfigure}
    % \hspace{5mm}
    \begin{subfigure}{0.32\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_yuguang/gap_imagenette_blend.pdf}
        \vspace{-5mm}
    \caption{BadNets-2}
    \end{subfigure}
    \vspace{-3mm}
    \caption{
    % \Yuguang{TBD: Change figure title!! 4 different Poisoning ratios, at guidance weight 5, 8 numbers in total.}
    Generation composition of BadNets-like trained SD on ImageNette. Settings are aligned with Fig.\,\ref{fig:generation_composition}. Generated images with trigger mainly stem from G2 (match the target prompt but contain the trigger) in low poisoning ratio (\textit{e.g.}, $p = 1\%$). While at a high poisoning ratio (\textit{e.g.}, $p = 10\%$), the proportion of G2 decreases, and trigger amplifications are shifted to G1.
    %(do not match the target promptly and contain the trigger). 
    This phenomenon is referred to as `\textbf{phase transition}' \textit{vs.} the poisoning ratio.
    % \SL{[what guidance weight?]} \SL{[G1 and G2 are not clear.]}
    }
    \label{fig:ratio_wrt_pr}
    \vspace{-6mm}
\end{wrapfigure}

==> sections/outline.tex <==
\Yuguang{Outline starts here.}

\section{Introduction}
  Considering to include the following paragraphs/topics
    \begin{enumerate}
        \item Briefly review the existing works of backdoor diffusion models from \href{https://arxiv.org/abs/2212.05400}{[backdoor diffusion papers]} \cite{chou2023backdoor} and point out their deficiencies and inappropriate assumptions (Attacker can not access to training pipeline!). Finally raise our question (motivation): "Can DMs be poisoned as simple as Badnet?" (\href{https://www.overleaf.com/project/646808062370deae1f2bb139}{link}).

    \SL{[Key research question to be answered in the paper like below:]}
    \begin{tcolorbox}[before skip=2mm, after skip=0.0cm, boxsep=0.0cm, middle=0.0cm, top=0.1cm, bottom=0.1cm]
        %\vspace*{1mm}
        \textit{\textbf{(Q)} Is there a theoretically-grounded and broadly-applicable method to improve approximate unlearning across different unlearning criteria?}
        %\vspace*{1mm}
    \end{tcolorbox}
        
        \item Our backdoor diffusion method, evaluation and challenges: How to perform backdoor attack on DMs? How do we differ from previous works? (poison data only)

        \SL{[You can emphasize one point here: Creating backdoored diffusion models remains a formidable challenge, as indicated by the current literature. E.g., It relies on modifications to training process/objective function/sampling process, or requires text prompt optimization etc.]}
        
        \item Application of our backdoor diffusion: Three case studies  (backdoor detection, data replication and backdoor defense). 

        \SL{[You can raise and focus on one point here: Backdoored diffusion models were only studied through the lens of backdoor attacks, with limited exploration of their potential benefits for enhancing backdoor defenses. Currently, there is a notable absence of studies delving into the inherent diffusion model properties, such as data memorization and the 'free' classification capacity of these models, to understand their implications for backdoor characteristics.]}

        \textbf{Remark:} We need a \textbf{Figure} in the Introduction to show the BackdoorDiff pipeline and the most significant experiment results (possibly together with the key technology). \SL{Please continue improving the figure (e.g., deliver the most significant messages/differences with existing works) and check Table 1 in \url{https://arxiv.org/pdf/2202.13711.pdf}. }
    \end{enumerate}

    % \begin{table}[htbp]
    % \resizebox{\linewidth}{!}{
    %     \begin{tabular}{c|ccc|cc|ccccc|c}
    %     \hline
    %     \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Treat Model} & \multicolumn{2}{c|}{Trigger Type} & \multicolumn{5}{c|}{Evaluation} & \multirow{2}{*}{Reference} \\ 
    %      &  \makecell{Training\\Data} & \makecell{Training \\ Process} & \makecell{Sampling} & Vision & Text & \makecell{Clean \\ Performance} & \makecell{Attack \\ Performance} & \makecell{Backdoor \\ Signature} & \makecell{Data \\ Replication} & \makecell{Diffusion\\Classifier} & \\ \hline
    %     BadDiff & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2212.05400.pdf}{(Chou et al., 2022)} \\
    %     TrojDiff & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2303.05762.pdf}{(Chen et al., 2023)} \\
    %     VillanDiff & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2306.06874.pdf}{(Chou et al., 2023)}\\
    %     Multimodal & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2305.04175.pdf}{(Zhai et al., 2023)}\\
    %     Rickrolling & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2211.02408v1.pdf}{(Struppek et al., 2022)}  \\ \hline
    %     Ours & \checkmark & & & \checkmark & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & This work \\
    %     \hline
    %     \end{tabular}
    % }

    \begin{table}[htbp]
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|ccc|ccccc|c}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Treat Model} &  \multicolumn{5}{c|}{Evaluation} & \multirow{2}{*}{Reference} \\ 
         &  \makecell{Training\\Data} & \makecell{Training \\ Process} & \makecell{Sampling} & \makecell{Clean \\ Performance} & \makecell{Attack \\ Performance} & \makecell{Backdoor \\ Signature} & \makecell{Data \\ Replication} & \makecell{Diffusion\\Classifier} & \\ \hline
        BadDiff & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2212.05400.pdf}{(Chou et al., 2022)} \\
        TrojDiff & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2303.05762.pdf}{(Chen et al., 2023)} \\
        VillanDiff & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2306.06874.pdf}{(Chou et al., 2023)}\\
        Multimodal & \checkmark & \checkmark & & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2305.04175.pdf}{(Zhai et al., 2023)}\\
        Rickrolling & \checkmark & \checkmark & & \checkmark & \checkmark & & & & \href{https://arxiv.org/pdf/2211.02408v1.pdf}{(Struppek et al., 2022)}  \\ \hline
        Ours & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & This work \\
        \hline
        \end{tabular}
    }
    
    \caption{Summary of the 5 existing works about injecting backdoor to diffusion model, and the proposed backdoor method. We list their attack assumptions (which parts of model training the attacker can access to) and the modality of trigger.}
    \end{table}
    


    \section{Related work}
    \begin{enumerate}
        \item Backdoor attack on DMs
        \item Data replication of DMs (\href{https://docs.google.com/spreadsheets/d/17Oi0M_qn0PdV4xkMTeem3P9qtHJdgmAfVmt14Uw0Zao/edit#gid=0}{link}) 
        \item Adversarial defenses using DMs? (\href{https://arxiv.org/pdf/2305.15241.pdf}{link}) \cite{chen2023robust}
        \SL{[You can focus on one point: To date, none of the defenses built upon diffusion models have been considered against backdoor attacks.]}
    \end{enumerate}

   \section{Problem statement}
    \begin{enumerate}
        \item 
        Existing backdoor attacks on diffusion models necessitate substantive modifications to the training procedure, which assumes that the adversary and the trainer are in fact an alliance. We think that their assumptions about the attacker's capabilities are too strong and ask the question: can backdoor attack diffusion models be as simple as Badnet? We focus on the Badnet setting because it requires no assumption on manipulating training objectives and diffusion processes. Thus it can be aligned with the backdoor attacks on the classification model.
        
        Threat Model: introduce the adversary's goal and capabilities to perform backdoor attack. 
        Backdoor attack types:   
        Inject blend-based trigger or patch-based trigger to p\% images and associate them to target labels.

        \SL{[You can highlight one point: We intend to examine the BadNet setting, the basic backdoor attacks for image classification, in diffusion models. The rationale is that this requires the least assumption on manipulating training objectives and diffusion processes.]}

        \item \SL{Diffusion processes and DM training.}

        \SL{Classifier-free diffusion and stable diffusion, prompt setting etc should be introduced here.}

        \SL{You can also mention the types of DMs focused on in the rest of the paper.}
        
        \item Definitions of the success of backdoor attack for \SL{image generation}. A successful attack should meet at least one of the following definitions while maintaining the ability to generate high-quality non target class images.
        \SL{[better to use concise and precise languages to describe the backdoor success criteria. This is very important.]}
         \SL{[Then, provide explanations and visual examples. A figure is needed here!]}
        \begin{enumerate}
            \item \SL{[Incorrectly generated images, misaligned with text prompt.]} Generate non-target class images condition on target class. The ratio of non-target class images should be more than the poison training data.
            \item \SL{[Harmfully generated images, even aligned with text prompt.]} Generate low quality target class images (e.g. generate target class images with trigger). Note that there are no target class images with triggers in poison training set.
        \end{enumerate} 


     

        
        \item \SL{\textbf{Problems of interest}. Please state problems that you want to study, and need to hook with the above preliminaries and the previous motivations.}
        \SL{Check the following paper, Sec. 3 of \url{https://arxiv.org/pdf/2111.01124.pdf}.}
        \SL{[Motivating results/examples could be considered here.]}
        \SL{[The above defined problems should correspond to the following sections of your study.]}
    \end{enumerate}  

    %\section{Attack performance}
    \section{\SL{Can DMs Be Backdoored As Easily As BadNets?}}

    \SL{[Focus on two scenarios: (1) DM is used as a generative model. (2) DM is used as a classifier. ]}

    \begin{enumerate}
        \item Evaluation metrics: \SL{[Confused with attack success criteria in Problem Statement section. Or you want to highlight `additional' metrics.]}
        \begin{enumerate}
            \item Trigger ratio of generated images, detected by a classifier specifically trained to detect the presence of triggers.
            \item Non-target images ratio of generated images condition on target class, detected by a clean classifier.
            \item MSE of generated trigger (How to evaluate the quality of blend-based trigger?)
            \item FID of generated images condition on non-target class. 
        \end{enumerate}
        \item Result: \SL{[Please consider a more informative paragraph title. E.g., trigger amplification is a key point and will be used for backdoor defense as well. Also, when can DMs be backdoored vs. poison ratio?]}
        \begin{enumerate}
            \item A grid figure visualizes the backdoor examples.
            \item A line chart shows the trigger raio and non-target class image ratio condition on target class.
            \item A histogram shows the FID score of generated samples.
        \end{enumerate}
        There are actually two graphs for each item corresponding to CIFAR10 and ImageNette.

        \SL{[In the end, you could have a summary of insights. Please check examples: Sec. 4 of \url{https://arxiv.org/pdf/2308.10110v1.pdf}, and Sec.\,4 of \url{https://openreview.net/pdf?id=JL6MU9XFzW}.]}
    \end{enumerate}

    \section{\SL{Defending Backdoor Attacks by Backdoored DMs}}

    \SL{[In this section, you should consider the following defense categories: (1) Trigger amplification of backdoored DMs could help detect backdoor attacks, without resorting to any `clean' data or models. (2) Low-poison ratio: The story could be different. The generated images by their own could be used to train a better classifier. Rationale? Since trigger amplification occurs mostly for generated images belonging to the target class. (3) The case of diffusion classifier?]}

    \begin{enumerate}
        \item Detection on generated data will be easier than on training data due to an amplification of trigger ratio.
        \item Detection methods: Introduce the two backdoor detection methods (\href{https://openreview.net/pdf?id=o0LFPcoFKnr}{SPC} and \href{https://openreview.net/pdf?id=S3D9NLzjnQ5}{Cognitive Distillation}) and more detection methods that we can use. 
        \item Result:
        \begin{enumerate}
            \item A line chart shows the mean of SPC value of (1) samples generated by backdoored DM (2) samples generated by clean DM (3) poison training data. The mean SPC value of (1) is the highest because DM amplifies trigger ratio.
            \item A line chart shows the mean of cognitive distillation value of (1) samples generated by backdoored DM (2) samples generated by clean DM (3) poison training data.
            \item Detect poison target class: a violin plot or box plot shows the cognitive distillation value distribution of  each class. The cognitive distillation value of the target class will be lower (indicating more likely to have a trigger) than other classes. (TODO compare with training data)
        \end{enumerate}
    \end{enumerate}

    \section{\SL{Explaining Backdoored Diffusion Models Through Data Replication Analysis}}

\SL{[What are the main insights you want to deliver and have each of them as a `paragraph'.]}

    Another major concern about diffusion models is data replication, which means that diffusion models generate images highly reminiscent of the training data, potentially leading to copyright concerns. Since our backdoor attack contaminates the training data of diffusion models, it raises a pertinent question: does a backdoor attack exacerbate data replication considering the mislabeled training data? Or can the attacker utilizes data replication to enhance the backdoor attack by injecting backdoor into different training data?
     
    In this section, we systematically delve into the intricate interplay between backdoor attacks and data replication. Our investigation gives a positive answer to the above questions and reveals a mutually reinforcing relationship where backdoor attacks can amplify the impact of data replication if we inject backdoor into the almost duplicate training data, and in turn, utilizing data replication can enhance the effectiveness of backdoor attacks. Furthermore, our study delves into the memory order of triggers and objects, shedding light on the underlying mechanisms that drive backdoor behaviors of diffusion model through the lens of data replication.

    \subsection{How to detect replication?}
    To align with previous works \cite{somepalli2023understanding}, we use the cosine similarity of the image SSCD features as the similarity score of the two images. The similarity between a generated sample and the training set is defined as the similarity between the generated sample and its top-1 match in the training data.
    
    
    \subsection{Backdoor for data replication}
    We find that the diffusion model can exhibit a more pronounced data replication under backdoor attacks, but the data replication effect is strongly correlated with which data we inject the backdoor into. Figure \ref{fig:dp-backdoor} shows a significant enhancement in data replication when we inject the backdoor into the most duplicate images in the training data. One possible explanation for this phenomenon is the narrowing of the class-conditional training set. In other words, in the backdoor training set, images within class A (not target class) but mislabeled to target class, are far less than correctly labeled class A images. This leads to a great difficulty in fitting the distribution of these mislabeled samples but fail to memorize the data point. Our finding echos the previous work  \cite{somepalli2023diffusion} which points out that a smaller training set leads to stronger data replication.
    
    \begin{figure}[htbp]
          \centering
          \includegraphics[width=\linewidth]{figures/dp_1.png}
          \caption{Data replication when inject backdoor to different kinds of images}
          \label{fig:dp-backdoor-outline}
    \end{figure}

    \subsection{Data for enhance backdoor attacks}
    From the adversary's perspective, the attacker can consciously utilize data replication to enhance the backdoor effect. Tab.\,\ref{tab:replication_amp} shows the ratio of mislabeled images generated by the backdoor diffusion model, the legend ``bd\_dup" means inject backdoor into the almost duplicate training samples, ``random" means inject backdoor randomly and ``no\_dup" indicated inject backdoor into the least duplicate images. Our experiment indicates diffusion model will generate more images that do not align with their respective prompts when the attacker injects the backdoor into more duplicate training data.

    % \begin{figure}[htbp]
    %     \centering
    %     \begin{subfigure}[b]{0.45\textwidth}
    %         \includegraphics[width=\textwidth]{figures/non_target_dup_badnet_pr0.05.png}
    %         \caption{poison ratio = 5\%}
    %         \label{fig:backdoor-dp-1-outline}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.45\textwidth}
    %         \includegraphics[width=\textwidth]{figures/non_target_dup_badnet_pr0.1.png}
    %         \caption{poison ratio = 10\%}
    %         \label{fig:backdoor-dp-2-outline}
    %     \end{subfigure}
    %     \caption{Ratio of mislabeled images generated condition on target prompt}
    %       \label{fig:backdoor-dp-outline}
    % \end{figure}

    % \begin{enumerate}
    %     \item  
    %     Replication help backdoor: Inject backdoor to duplicated training data (or training data which are easier to memorize) can enhance the backdoor effect.  

    %     Result: A line chart shows the ratio of non target images when we inject backdoor to (1) most duplicated data (2) randomly selected data (3) least duplicated data.
    %     \item \SL{This is the angle `Backdoor for data replication.'}
    %     Backdoors exacerbate data replication: Replication becomes more severe under backdoor attack if we inject backdoor to duplicated training data (or training data which are easier to memorize).
        
    %     Result: A density plot of the similarity score distribution when we inject backdoor to (1) most duplicated data (2) randomly selected data (3) least duplicated data.

    %     \item The triggers on the generated samples can be considered as a local content replication. 
    %     \SL{This is the angle of `trigger amplification.'}
    %     And replicating trigger is easier than replicating non target class content. We need a figure showing the trigger ratio and non target class image ratio over different poison ratio.
    % \end{enumerate}

    \section{Backdoor Defense}
    \SL{[This section should be combined with Sec. 5.]}
    \begin{enumerate}
        \item Train classifier on generated data because DM generate less non target class images when poison ratio is low. 

        Result: A table shows the accuracy and attack success rate of classifier trained on generated data v.s. poison training data.
        \item Classify by DM and defend backdoor by filtering out the top p\% pixels errors. \Yuguang{In other words, this is an extension application of the paper Diffusion Classifier \cite{li2023your} on backdoor dataset.}
        
        Result: A table shows the accuracy and attack success rate of DM classifier over different filer thresholds.
        \item \Yuguang{Can we have an analysis over this two phase phenomena? Following \textbf{Exp1.2}, is there a way for us to determine such a threshold for the mitigation versus the amplification for different diffusion models?}
    \end{enumerate}
     
    \section{Conclusion}

